Towards Point-Free Spacetimes

In this thesis we propose and study a theory of ordered locales, a type of point-free space equipped with a preorder structure on its frame of opens. It is proved that the Stone-type duality between topological spaces and locales lifts to a new adjunction between a certain category of ordered topological spaces and the newly introduced category of ordered locales. As an application, we use these techniques to develop point-free analogues of some common aspects from the causality theory of Lorentzian manifolds. In particular, we show that so-called indecomposable past sets in a spacetime can be viewed as the points of the locale of futures. This builds towards a point-free causal boundary construction. Furthermore, we introduce a notion of causal coverage that leads naturally to a generalised notion of Grothendieck topology incorporating the order structure. From this naturally emerges a localic notion of domain of dependence, which is generally distinct from the traditional notion in spacetimes.

==> sections/ch0-introduction.tex <==
\section{Overview of pointfree topology and mereology}
foo

==> sections/geometry.tex <==
\section{Pseudo-Riemannian geometry}
\label{section:pseudo-riemannian geometry}
In this section we provide the background material that is necessary to formulate the precise definition of a \emph{spacetime} (\cref{definition:spacetime}). The main ingredients are the notions of a \emph{smooth manifold}, and that of a \emph{metric}.

\begin{definition}
	\todo{Smooth manifolds.}
\end{definition}

\begin{definition}
	\todo{(Co)Tangent bundles.}
\end{definition}

\begin{definition}
	\todo{Metrics.}
\end{definition}

==> sections/journal.tex <==
\section{Pointless thoughts}
\paragraph{19-05-2023.} As discussed also in \cref{section:literature draft}, we should make a convincing motivation to study pointfree spaces. It would be nice to give a fun overview of the landscape of such theories. 

The best starting point would be to begin with topological spaces $S$ versus locales $X$. To highlight the benefits of locales over ``pointy'' spaces, we should probably consult \cite{johnstone1983PointPointlessTopology}. Further, it would be fun to mention things like the Banach-Tarski paradox. I remember someone on MathOverflow pointing to the following article: \cite{simpson2012MeasureRandomnessSublocales}. Some stuff that comes to mind:
	\begin{enumerate}
		\item arbitrary intersections of dense sublocales are dense. What does this entail, why is it special, and why does it \emph{not} hold for spaces?
		\item products being better behaved;
		\item measure theoretic benefits, Banach-Tarski paradox, etc.?
	\end{enumerate}

\paragraph{22-05-2023.} Reading the appendix of \emph{Orthogonality and Spacetime Geometry} by Goldblatt (1987), and there's a nice little history of axiomatisations of Minkowski space. They mention the book by A.A.Robb,\emph{ A Theory of Time and Space} (1914). And they derive a result by Alexandrov-Zeeman on causal automorphisms in relation to Lorentz transformations. 

In addition to a history of pointfree spaces, it would be nice to also give an history of spacetimes and their axiomatisations. 

\paragraph{22-06-2023.} The following table is good to discuss in the introduction of the thesis to showcase the motivation from tensor topology. 

\begin{table}[h]
	\centering
	\begin{tabular}{l|l|l}
		\textbf{Pointy}      & \textbf{Point-free}& \textbf{Categorification} \\ \hline
		Ordered spaces     & {\color{Green}Ordered locales}   & ???              \\ \hline
		Topological spaces & Locales           & SMC             
	\end{tabular}
\end{table}

\paragraph{23-06-2023.} Using laws like~\eqref{axiom:L}, can we develop a theory of \emph{``ordered (semi)lattices''}? Can we get a duality? What if we just use the localic cones without reference to $\Leq$?

\paragraph{04-07-2023.} Some authors have argued for different topologies on spacetime manifolds, see e.g. \cite{hawking1976NewTopologyCurved,gobel1976ZeemanTopologiesSpacetimes}. (We should refer to older literature by Alexandrov and Zeeman, but can't be bothered finding the references now.) There are arguments against this, too: \cite{heathcote1988ZeemanGobelTopologies}. It seems most of our discussions of spacetimes in the setting of ordered locales is heavily predicated on some strong topological connections between $I^\pm$ and $J^\pm$, and hence hinge heavily on the use of the manifold topology. In the thesis we should say some words on this choice, and perhaps even investigate the ordered locale structure of the other topologies mentioned.

\paragraph{12-07-2023.} I think the proof of Lemma~6.4 in \cite{heunenSchaaf2023OrderedLocales} does not work in general, but only for locales satisfying the extra axiom (P)! This needs to be fixed. Luckily, it doesn't actually destroy the main result.

Actually, if $\delta$ is the inverse of the counit $\epsilon_X\colon \loc(\pt(X))\to X$, it seems even true that $\delta$ is monotone if and only if (P) holds. Interesting.

\begin{lemma}
	For a spatial ordered locale $X$, the inverse of the counit $\delta$ is monotone if and only if axiom (P) holds.
\end{lemma}
\begin{proof}
	We now know that axiom (P) is sufficient to prove that $\delta$ is monotone, namely calculate:
		\[
			\Up \delta^{-1}(\pt(U)) = \Up U = \delta^{-1}(\pt(\Up U)) \subseteq \delta^{-1}(\Up\pt(U)).
		\]
	The last inclusion is due to (P), namely since $U\Leq \Up U$ implies $\pt(U)\Leq\pt(\Up U)$, which in particular means $\pt(\Up U)\subseteq \up\pt(U)$, so by taking interiors we get $\pt(\Up U)\subseteq \Up \pt(U)$.
	
	Conversely, suppose that $\delta$ is monotone. It suffices to show that $\pt(\Up U)\subseteq \Up\pt(U)$. Using that $\delta$ is monotone gives $\Up U = \Up \delta^{-1}(\pt(U))\subseteq \delta^{-1}(\Up \pt(U))$, and since $\delta$ is the inverse of $\epsilon_X$ this implies $\pt(\Up U)\subseteq \Up\pt(U)$, as desired.
\end{proof}

Wow! OK this is nice, but does it not diminish the power of our result slightly? We're sort of already starting with locales that will live in the fixed points (save those that are non-spatial)\ldots

\paragraph{22-07-2023.} I was chatting to Jan Głowacki at QPL a few days ago, and he was quite enthusiastic about the domains of dependence and deterministic sheaf idea. He suggested that $\Cov^\pm$ should actually define Grothendieck topologies on the Kleisli categories induced by $\Up$ and $\Down$. This would be quite nice! 

So, the idea is that $(V_i)_{i\in I}\in \Cov^-(U)$ iff $\bigvee_{i\in I} V_i$ covers $U$ from the past. Thus we can see it as a family of morphisms $(V_i\to \Down U)_{i\in I}$. Of course, these are just arrows $V_i\to U$ in the Kleisli category of the localic past $\Down$. Let's denote this by $\Opens X_{\down}$. Then does this define a Grothendieck topology on $\Opens X_{\down}$? This is something to check. Thanks, Jan, for the suggestion! I'm also very grateful to JSPL and Bert Lindenhovius and Rui Suares Barbosa for showing enthusiasm about the talk afterwards, among other people.

Update: confident that this defines a Grothendieck topology on the Kleisli category. However it seems strange to interpret sheaves on this category as data living ``on'' opens. Namely an arrow $U\to V$, which is really an inclusion $U\sqleq \Down V$, is associated to a function $FV\to FU$. How do we interpret this? In any case, the natural functor $\Opens X \to \Opens X_{\Down}$ into the Kleisli category preserves covers. This is half of the definition of a morphism of sites. Unfortunately, the other one (being ``covering-flat'') is not satisfies, since that would correspond to the localic cones preserving meets (which they don't). 

\paragraph{02-08-2023.} At ACT I've been learning about \emph{Markov categories}. One way to get a Markov category is through the Kleisli category of a so-called \emph{probability monad}. Apparently valuations on locales determine such a monad \cite{vickers2011MonadValuationLocales}, and hence their Kleisli category determines a Markov category, a sort of probabilistic version of locales and their morphisms. There is also a notion of valuation on topological spaces, that form a probability monad \cite{fritz2021ProbabilityValuationsHyperspace}. My question: does the duality between spaces and locales lift to these Kleisli categories, so that we get a sort of probabilistic Stone duality:
	\[
		%https://q.uiver.app/#q=WzAsNCxbMCwxLCJcXFRvcCJdLFswLDAsIlxcS2xlaXNsaShWKSJdLFsxLDAsIlxcS2xlaXNsaShcXG1hdGhmcmFre1Z9KSJdLFsxLDEsIlxcTG9jIl0sWzAsMSwiIiwwLHsib2Zmc2V0IjotMn1dLFsxLDAsIiIsMCx7Im9mZnNldCI6LTJ9XSxbMywyLCIiLDAseyJvZmZzZXQiOi0yfV0sWzIsMywiIiwwLHsib2Zmc2V0IjotMn1dLFswLDMsIlxcTG9jIiwwLHsib2Zmc2V0IjotMn1dLFszLDAsIlxccHQiLDAseyJvZmZzZXQiOi0yfV0sWzEsMiwiPyIsMSx7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6InNxdWlnZ2x5In0sImhlYWQiOnsibmFtZSI6Im5vbmUifX19XSxbNCw1LCIiLDAseyJsZXZlbCI6MSwic3R5bGUiOnsibmFtZSI6ImFkanVuY3Rpb24ifX1dLFs2LDcsIiIsMCx7ImxldmVsIjoxLCJzdHlsZSI6eyJuYW1lIjoiYWRqdW5jdGlvbiJ9fV0sWzgsOSwiIiwxLHsibGV2ZWwiOjEsInN0eWxlIjp7Im5hbWUiOiJhZGp1bmN0aW9uIn19XV0=
		\begin{tikzcd}
			{\Kleisli(V)} & {\Kleisli(\mathfrak{V})} \\
			\Top & \Loc
			\arrow[""{name=0, anchor=center, inner sep=0}, shift left=2, from=2-1, to=1-1]
			\arrow[""{name=1, anchor=center, inner sep=0}, shift left=2, from=1-1, to=2-1]
			\arrow[""{name=2, anchor=center, inner sep=0}, shift left=2, from=2-2, to=1-2]
			\arrow[""{name=3, anchor=center, inner sep=0}, shift left=2, from=1-2, to=2-2]
			\arrow[""{name=4, anchor=center, inner sep=0}, "\loc", shift left=2, from=2-1, to=2-2]
			\arrow[""{name=5, anchor=center, inner sep=0}, "\pt", shift left=2, from=2-2, to=2-1]
			\arrow["{?}", squiggly, no head, from=1-1, to=1-2]
			\arrow["\dashv"{anchor=center}, draw=none, from=0, to=1]
			\arrow["\dashv"{anchor=center}, draw=none, from=2, to=3]
			\arrow["\dashv"{anchor=center, rotate=-90}, draw=none, from=4, to=5]
		\end{tikzcd}?
	\]
There is a straightforward assignment $V(S)\to \mathfrak{V}(\loc(S))$, but there should also be an assignment $\mathfrak{V}(X)\to V(\pt(X))$, which seems more difficult. There are also some subtleties about the real numbers that are pointed out in \cite{vickers2011MonadValuationLocales} but that I'm too ignorant to understand.


(Something else I don't understand is the difference between valuations on locales, and so-called measurable locales \cite{pavlov2022GelfandtypeDualityCommutative}. Is it like the difference between measure spaces and measurable spaces?)

Given sufficiently well-behaved natural maps $V\to \mathfrak{V}\circ \loc$ and $\mathfrak{V}\to V\circ \pt$, can we define functors between $\Kleisli(V)$ and $\Kleisli(\mathfrak{V})$? Of course, on the objects we want to apply the functors $\loc$ and $\pt$. So we want to define a functor $\loc\colon \Kleisli(V) \to \Kleisli(\mathfrak{V})$ by $S\mapsto \loc(S)$, and sending an arrow $S\to T$, which is really a continuous function $g\colon S\to V(T)$, to a map of locales $\loc(S)\to \mathfrak{V}(\loc(T))$. First, we get $\loc(g)\colon \loc(S)\to \loc(V(T))$. So what we really need is some natural map $\loc\circ V \to \mathfrak{V}\circ \loc$? Similarly, we want to send an arrow $f\colon X\to\mathfrak{V}(Y)$ in $\Loc$ to an arrow $\pt(X)\to V(\pt(Y))$ in $\Top$. We get $\pt(f)\colon \pt(X) \to \pt(\mathfrak{V}(Y))$, and we need to turn this into a continuous function $\pt(X) \to V(\pt(Y))$. That this is possible is actually motivated by remarks in \cite{vickers2011MonadValuationLocales}, where it is mentioned that the \emph{points} of $\mathfrak{V}(Y)$ are actually the valuations on $Y$.

To summarise, we need to construct two canonical natural transformations:
	\[
		\loc\circ V \longrightarrow \mathfrak{V}\circ \loc
		\qquad\text{and}\qquad 
		\pt\circ \mathfrak{V}\longrightarrow V\circ \pt.
	\]
Is this enough for the adjunction to lift? (Tried working some stuff out on paper; I think we need more conditions to get functors.)

Update: thanks to Paulo for some nice discussions. He explained to me how the category $\Kleisli(V)$ is actually equivalent to the Kleisli category of $V$ restricted to \emph{sober} spaces. In particular, $V(S)$ is always sober. In this sense, valuations really are a localic thing. The adjunction above therefore is on the face of it less interesting than I initially thought. Lifting $\loc\dashv\pt$ to the Kleisli categories therefore would come down to proving that $\Kleisli(V)$ is a nice subcategory of $\Kleisli(\mathfrak{V})$. I'm not sure if it's worth going into that now; especially since I only have about 4 months to finish my thesis.

\paragraph{14-08-2023.} What is the structure of the set of preorders on a locale that make it into an ordered locale? Do we have meets and joins? This would allow us to have some nice universal constructions, perhaps.

Since we're just getting started, here is a list of questions we can get started on:
	\begin{enumerate}[label = (\arabic*).]
		\item continue studying indecomposable past sets in ordered locales:
			\begin{enumerate}
				\item we now know there are spatial ordered locales without IPs, and locales without points but with IPs. Clean characterisation of existence of IPs along the lines of \cite[Lemma~3.3]{geroch1972IdealPointsSpaceTime}? Characterise IPs in terms of ``points'' $1\to X$, but the domain replaced by some suitable shape?
				\item alternatively: IPs as points in $(\im(\Down),\sqgeq)$;
				\item figure out if we can characterise causal continuity (and other causality conditions) using IPs;
				\item have another go at distinguishing between PIPs and TIPs abstractly (using lattice theory?);
			\end{enumerate}
		\item sheaves on ordered locales:
			\begin{enumerate}
				\item figure out if our notion of coverage in an ordered locale gives (under reasonable assumptions, e.g. in a spacetime) the intuition that every curve needs to pass through a region;
				\item Grothendieck topology on the Kleisli category (of a localic cone);
				\item ``$D$-sheaves'' for $D$ a monad (and relation to previous point);
				\item examples (automata, wave equation, dynamical systems);
			\end{enumerate}
		\item internal preorders in the category of locales:
			\begin{enumerate}
				\item clean characterisation of~\eqref{axiom:LV} in terms of $\Leq$;
				\item translate internal preorder in $\Loc$ to $\Leq$?
			\end{enumerate}
		\item induced order on sublocales:
			\begin{enumerate}
				\item this allows us to talk about the future/past of e.g. closed or compact sublocales;
				\item can we use this to formulate other causality conditions, such as global hyperbolicity?
			\end{enumerate}
	\end{enumerate} 

Here is something important that I found while reading \cite[p.8]{marolf2003NewRecipeCausala}: namely, there exist causally continuous spacetimes that admit an IP $P$ such that $C^+(P)$ is \emph{not} an IF! This is apparently proven in \cite{rube1990ExampleNontrivialCausally}, but I haven't been able to find a \texttt{pdf}. Hence our localic generalisation saying $C^+$ takes IPs to IFs cannot be correct, and needs to be sharpened.

See also \cite{garcia-parrado2005CausalStructuresCausala} for a somewhat more modern overview of boundary constructions, and some sections on IPs.

\paragraph{15-08-2023.} Found a \texttt{pdf} of \cite{rube1990ExampleNontrivialCausally}. It's only a two page paper, but the upshot is that there exists a causally continuous spacetime with a TIF whose common past is non-empty but \emph{not} an IP. So our current best guess is that $M$ is reflecting iff $C^\pm$ preserve PIP/Fs.

Another thought: \cite{vickers2011MonadValuationLocales} constructs $\mathfrak{V}X$ as a locale whose \emph{points} are the valuations on $X$. Similarly, should we think of the causal completion of an ordered locale $X$ as one whose \emph{points} are the IP/IFs of $X$?

\paragraph{17-08-2023.} First day back at the office, and just got back from lunch after a meeting with Chris. It was good to see people! I made some headway on the problem about viewing IPs as points yesterday. This is described a little bit in the Overleaf with Prakash. See there for details. The new insight we had during the meeting is that also the Kleisli category $\Kleisli(\Down)$ of the localic past cone forms a frame! This is interesting, since it is this frame that $\CovLeq^-$ defines a Grothendieck topology on. Is this the canconical covering defined by the frame structure?

\paragraph{23-08-2023.} This week has been really frustrating. I've been super confused delving into all the lattice theoretic details, and it's just not budging. 

I just hopped on here to record a remarkable result: \cite[p.~283]{johnstone1982StoneSpacesa}. This says that if $A$ is a distributive complete lattice, then it is completely distributive if and only if the interval topology is Hausdorff. This sounds an awful lot like the characterisation of strongly causal spacetimes in terms of the Alexandrov topology being Hausdorff.

\paragraph{31-08-2023.} I was thinking about the irrational torus as an example of an ordered space, and whether it has open cones. I still don't know, but this got me thinking about quotients of ordered spaces. We know actually very little about $\OrdTop$, and $\OrdTop_\OC$. This should probably be rectified. Are they topological over $\Ord$? 

\paragraph{08-09-2023.} We should find a counter-example of an ordered locale that does not satisfy~\eqref{axiom:LV}.

\paragraph{12-09-2023.} We should look at ``coprime decomposition'' theorems from lattice theory, and see what they tell us about IPs.

\paragraph{13-09-2023.} In \cite{minguzzi2019LorentzianCausalityTheory} on page~118, before Section~4.3, they mention something we should think more about. Namely Minguzzi argues for the use of a \emph{closed} order on the spacetime, given by $K$ (the smallest transitive closed relation containing the causality relation) or the Seifert relation $J_S$. Abstractly, Minguzzi develops this in \url{https://arxiv.org/abs/1709.06494}. He then claims that both order and topology are actually captured by something else: \emph{quasi-uniformity}. What is this, and does it generalise naturally to the localic setting? A \emph{quasi-uniformity} $\mathcal{U}$ on a set $S$ is something like a filter in the powerset of $S\times S$, i.e. containing relations on $S$, that are all reflexive, and satisfy something like a weaker form of transitivity. This has apparently already been generalised to frames: \emph{Entourage uniformities for frames}, by P. Fletcher and W. Hunsaker. Keep in mind the existence of a closed reflexive relation implies Hausdorffness. (Note added later: whereas every topology comes from a quasi-uniformity, I think not every ordered space comes from a quasi-uniformity.)

\paragraph{14-09-2023.} In \emph{The Causal Boundary of Spacetimes Revisited} by José L. Flores they show that, using a completion procedure for ``chronological sets,'' it is possible to characterise global hyperbolicity and causal continuity. This is promising for us, too. See their Theorems~9.1 and~9.3.

\paragraph{21-09-2023.} We should reference \cite{priestley1972OrderedTopologicalSpaces}. She calls spaces with open cones ``I-spaces.''

\paragraph{22-09-2023.} Today, I think we solved the discrepancy of localic causal completions and IP/IFs. Since the localic cones of a spacetime are severely regular (\cref{lemma:chronological cone of double negation,lemma:chronological cones are regular opens}) it means that we can think of IPs equivalently as ``complements'' of IPs. The IPs are coprimes $P\in \im(\Down)$, and hence induce \emph{primes} $\neg P\in \im(\Up)$. But the primes of $\im(\Up)$ are roughly the \emph{points} of $\Ideals(\im(\Up))$. Since Heyting negation is \emph{anti}-monotone, this also corrects an error in the direction of the causal completion. Namely, we first thought of $\Ideals(\im(\Down))$ as a \emph{future} completion, since the IPs live in $\im(\Down)$ and IPs are used as future ideal points. But with this new insight it becomes clear that $\Ideals (\im(\Down))$ should be seen as a \emph{past} completion. The connection to IFs arises by taking Heyting negations, and this gives a correct ordering on the points. Details should be worked out soon! But this makes me very happy.

\paragraph{25-09-2023.} If the domains of dependence $D^\pm$ are monads on $\Opens X$, then what is their induced order $\Leq$?

Also, now that we have a better candidate for the past boundary completion of $X$, namely $X^\triangledown$, can we make a definition of global hyperbolicity? According to \cite[Section~4]{szabados1988CausalBoundaryStrongly} a spacetime $M$ is globally hyperbolic if and only if $C^+(P)=\varnothing$ for every TIP $P$. How do we translate that into primes of $\im(\Down)$? First recall that we have a proof in the Overleaf that if $P$ is a PIP then $C^+(P)\neq\varnothing$. So a spacetime is globally hyperbolic precisely when, for every IP $P$, $C^+(P)=\varnothing$ if and only if $P$ is a TIP. How can we state this in a locale? First we need to find an analogue of $C^+(P)=\varnothing$, but stated in terms of $\neg P$. Note that in a spacetime $C^+(P)\sqleq \neg P$. 

(Later in the day:) Some more insights. If we start with a space $S$, then the topology of $\pt(S^\triangledown)$ will be very different from that of $S$. There will be an order-isomorphism of $S$ to the image of $S\to \pt(S^\triangledown)$, but this will definitely \emph{not} be a homeomorphism. Take for instance $S=(\mathbb{R},\leq)$. Then $\mathbb{R}^\triangledown$ will only have opens of the form $(-\infty,a)$, so there is no way $\mathbb{R}$ embeds order-homeomorphically into $\mathbb{R}^\triangledown$. 

A potential solution is to adopt a strategy as first proposed by \cite{budic1974CausalBoundariesGeneral} and later used in \cite{szabados1988CausalBoundaryStrongly}, where for the completion one takes \emph{pairs} of IPs and IFs. Localically, this means instead of studying the frame $\im(\Down)$, we want to somehow combine $\im(\Up)$ and $\im(\Down)$. These two frames contain enough information to recover the original ``topology,'' at least as soon as the locale is \emph{strongly causal}. Namely, an ordered locale $X$ is strongly causal if and only if $\im(\Up)\times\im(\Down)\to \Opens X: (\Up U,\Down V)\mapsto \Up U\wedge \Down V$ is a surjection. I am pretty sure that this, in turn, holds if and only if the similar map of frames $\im(\Up)\oplus\im(\Down)\to \Opens X: \Up U\oplus \Down V\mapsto \Up U\wedge \Down V$ is a surjection (cf. \cite[Proposition~IV.5.2(5)]{picado2012FramesLocalesTopology}). Hence $X$ is strongly causal if and only if it is a sublocale of $X^\triangleup \times X^\triangledown$. The idea is then to take the points of $X^\triangleup \times X^\triangledown$ to recover the ideal points. But $\loc\dashv \pt$, so $\pt$ preserves limits, so $\pt(X^\triangleup\times X^\triangledown)\cong \pt(X^\triangleup)\times \pt(X^\triangledown)$, so at least in the spacetime case (or more generally the ``regular cone'' case) this is just the product of the set of IPs and IFs of $X$. But they need to be related in some sense, whereas now they are treated disjointly. So perhaps we need a factorisation of sublocales $X\to \overline{X}\to X^\triangleup\times X^\triangledown$, such that $\pt(\overline{X})$ will be something like pairs of IPs and IFs that obey the ``Szabados'' relation \cite{szabados1988CausalBoundaryStrongly} (cf. \cite{marolf2003NewRecipeCausala}).

\paragraph{26-09-2023.} A nice quote:
	\begin{quote}
		Topology is one extreme, where spaces are spaces of points, and, oh, in passing, they are glued together in some way.
		
		Locale theory is another extreme, where you recognize a space as a big amount of glue, and, oh, in passing, that glue sometimes connects infinitesimal things called points.
	\end{quote}
From \url{http://projects.lsv.ens-cachan.fr/topology/?page_id=1251}. I should get started working on the presentation for next Thursday!

\paragraph{27-09-2023.} Here are some papers we should check out to compare our work to the mereological theories of spacetime: \url{https://arxiv.org/abs/2004.14755} and \url{https://link.springer.com/article/10.1007/s10670-010-9262-y}.

I have been thinking about sublocales of $X^\triangleup\times X^\triangledown$, given by the coproduct frame $\im(\Up)\oplus \im(\Down)$. (Because: the points of this locale for a spacetime are exactly the pairs $(P,F)$ of IPs and IFs.) This got me thinking about Steve Vickers' prompt about thinking of ordered locales as sublocales of $X\times X$. It would be nice to at least have a relation between such things and our ``external'' definition using $\Leq$. For instance, if $j\colon R\rightarrowtail X\times X$ is a sublocale, can we fabricate an order $\Leq$ on $\Opens X$? Well, we get a map of frames $j^{-1}\colon \Opens X\oplus \Opens X\to \Opens R$. So we can try to define $U\Leq_R Y$ if and only if $j^{-1}(U\oplus V)=R:=\top_R$, the top element in $\Opens R$. At least this gives axiom~\eqref{axiom:V}: if $U_i\Leq_R V_i$ then $j^{-1}(U_i\oplus V_i)= R$, so
	\[
		R=\bigvee R = \bigvee j^{-1}(U_i\oplus V_i) 
		=
		j^{-1}\left(\bigvee (U_i\oplus V_i)\right)
		\stackrel{??}{=}
		j^{-1}\left(\bigvee U_i\oplus \bigvee V_i\right),
	\]
and hence suggesting $\bigvee U_i\Leq_R\bigvee V_i$. (Note: here I'm really playing fast-and-loose with the coproduct. The actual construction of coproducts of frames is more involved, so this might not be right.) Presumably, the fact that $R$ is reflexive and transitive (in a suitable sense) can be translated into $\Leq$ being a preorder. Reflexivity should be easy enough to check. First, by universality of the product, we can write $j = (s,t)$ for some maps $s,t\colon R\to X$. Of course, $s$ and $t$ are just $j$ followed by the respective projections. Then, according to the \href{https://ncatlab.org/nlab/show/preordered+object}{$n$Lab}, $R$ being reflexive means roughly that there exist a map $\rho\colon X\to R$ that is a section of both $s$ and $t$, i.e. $s\circ \rho =\id_X = t\circ \rho$. Does this imply $U\Leq_R U$? We claim that $R$ is reflexive according to this definition if it contains, as a subobject, the diagonal $\delta\colon X\to X\times X$. Recall \cite[Proposition~IV.5.2]{picado2012FramesLocalesTopology} that $\delta^{-1}(U\oplus V)= U\wedge V$. That $R$ contains $\delta$ means there is a map of locales $\rho\colon X\to R$ such that $j\circ\rho = \delta$. Projecting to components certainly implies that $s\circ \rho =\id_X$, since $(\pr_1 \circ \delta)^{-1}(U) = \delta^{-1}(U\oplus X) = U\wedge X = U$. So I believe it. But does it give reflexivity for $\Leq_R$? I get the feeling that a better definition is $U\Leq_R V$ iff $j^{-1}(U\oplus V)\neq\varnothing$. The proof above for~\eqref{axiom:V} will still work. Anyway, can we prove $j^{-1}(U\oplus U)\neq\varnothing$? We just know $(j\circ \rho)^{-1}(U\oplus V) = \rho^{-1}(j^{-1}(U\oplus V)) = U\wedge V $. Not sure. Note that $j^{-1}(U\oplus V) \neq \varnothing$ iff $j^{-1}(U\oplus V)\not\sqleq \varnothing$ iff $U\oplus V\not\sqleq j_\ast(\varnothing)$, since $j^{-1}\dashv j_\ast$. Just some observations; maybe let's continue this on paper.

\paragraph{29-09-2023.} A locale $X$ is strongly causal iff $X\to X^\triangleup\times X^\triangledown$ is a sublocale. But a spacetime is actually strongly causal iff its topology agrees with the Alexandrov topology, meaning that its topology is generated by opens of the form $I^+(x)\cap I^-(y)$. This seems like a significantly stronger condition, at least for locales. The analogue would be something like: $X$ is a sublocale of some suitable locale of IFs and IPs. Can we make a locale out of the IFs of $X$? The prime elements of $\im(\Down)$ certainly form a poset, simply with inclusion $\sqleq$. In a locale with regular cones, the IFs are in bijective correspondence with the prime elements of $\im(\Down)$. 

Also, we should frame a notion of ``completeness'' for ordered locales that generalises the idea that every timelike geodesic has an endpoint. Of course, we need to do this without using curves. Something like: no TIPs exist? But we still don't have any way to classify TIPs vs PIPs.

\paragraph{06-10-2023.} During meeting with Chris yesterday, we thought for a bit about what the ``completion'' $\overline{X}$ of an ordered locale $X$ should satisfy, as a universal property. The point of a completion of a spacetime is that it adds the endpoints to all geodesics/timelike curves. Of course, the curves that have an endpoint are just the points of the spacetime. The singularities are exactly the would-be endpoints of geodesics that don't have a limit in the actual spacetime. The order-theoretic generalisation of these ideas might be to make the causal order $\leq$ of $\pt(X)$ into a dcpo. In other words, we want an order-homeomorphic inclusion $\pt(X)\hookrightarrow \pt(\overline{X})$, but the causal order of $\pt(\overline{X})$ should be a dcpo: all directed joins(/meets) should exist. Or perhaps weaker: all chains should have a ``limit.''

STAMP talk didn't go super well. I'm actually quite disappointed, I shouldn't have procrastinated so much on the prep. There was technical difficulties with the Zoom at the start, and a lot of questions in the middle of the talk, and frankly I way underestimated how long it would take to write things on the blackboard. I had to skip a few sections, and I felt like I was just kind of rambling through the whole thing. I was glad with the engagement though, people were asking questions and afterwards spent chatting for about 30 minutes to some people who were interested.

\paragraph{27-10-2023.} Robert Booth asked me ``what we can do'' with our localic formulation of spacetime. There are the standard answers: ``well, the right notion of \emph{space} should really be \emph{locale}, so your spacetimes should be locales.'' Then what we are doing: ``using lattice-theoretic language, it is really elegant to describe singularities and causal boundaries.'' But can we say more? Spacetimes are, in particular, locally compact Hausdorff, so they will enjoy some nice topological properties. Such as: complete regularity. 

This notion has a localic generalisation, e.g. at \cite[\S V.5.7.1]{picado2012FramesLocalesTopology}. The condition can be phrased as saying that any element of the frame of opens can be written as the join over the elements that are \emph{completely below} it. To explain what this means, we need some notation. In a frame, write $a\ratherbelow b$, and say $a$ is \emph{rather below} $b$, if $\neg a\vee b = \top$. Equivalently, if there exists $c$ with $c\wedge a =\bot$ and $c\vee b = \top$. A locale is called \emph{regular} if every element can be written as the join of elements that are rather below it:
	\[
		U = \bigvee\{ V\in \Opens X: V\ratherbelow U\}.
	\]
See \cite[Section~V.5]{picado2012FramesLocalesTopology}. For spaces, this notion coincides with the classical definition \cite[\S V.5.3]{picado2012FramesLocalesTopology}. Some nice things happen: for instance the epimorphisms in the category of regular locales are precisely the \emph{dense} maps of locales.

Further, $a$ is \emph{completely below} $b$, $a\completelybelow b$, if there is a family $(a_r)_{r\in\mathbb{Q}\cap [0,1]}$ indexed by rational numbers $r\in [0,1]$ such that: $a_0 = a$, $a_1 =b$, and $a_r\caus a_s$ for $r< s$. For spaces, this notion is analogous to the classical definition \cite[\S V.5.7.1]{picado2012FramesLocalesTopology}. Apparently, $\completelybelow$ is the largest interpolative relation contained in $\ratherbelow$. The intuition isn't quite so clear yet.

What are the nice properties of (completely) regular locales? For one, according to \cite[Section~VII.4]{picado2012FramesLocalesTopology}, they are the locales for which you can do a point-free Stone-\v{C}ech compactification. They do this by refining the ideal construction $\Ideals(X)$ of a locale. Instead they use \emph{regular ideals}: an ideal $I\subseteq \Opens X$ is called \emph{regular} if for every $U\in I$ there exists $V\in I$ such that $U\completelybelow V$. By \cite[\S VII.4.2]{picado2012FramesLocalesTopology} the set $\RegIdeals(\Opens X)$ is a subframe of $\Ideals(\Opens X)$, and hence defines a regular locale. In $\Loc$, you get a map of locales $\Ideals(X)\to \RegIdeals(X)$. By \cite[\S VII.4.2.3]{picado2012FramesLocalesTopology}, if $X$ is completely regular, then so is $\RegIdeals(X)$. So in the category of completely regular locales, there is a compactification $X\to \RegIdeals(X)$. This is nicer than the $\Ideals(X)$ construction, since now if $X$ is already compact, then $X\cong \RegIdeals(X)$.

\paragraph{17-11-2023.} It's been a while since I wrote here. But I had the idea that we shouldn't just be looking in the relativity literature for causal boundary completions. Probably in the ordered topology literature there exists such a thing as an ordered compactification. These might prove insightful for our purposes!

In particular I'm looking at \emph{A New Ordered Compactification}, D.C. Kent, 1993 and \emph{Compactifications of ordered topological spaces}, T. McCallion, 1972. The latter uses the notation $[x,\to ] = \up\{x\}$, which is charming.

Later in the day: the ideas there seem quite promising. They also appear in \emph{Wallman's Type Order Compactification}, T.H. Choe and Y.S. Park, 1979. They apparently introduced the notion of a \emph{bifilter}: a pair of filters (in our notation) $\calF\subseteq \im(\Up)$ and $\calP \subseteq\im(\Down)$ with the property that:
	\[
		\forall F\in \calF \forall P\in\calP: F\wedge P\neq\varnothing.
	\]
The idea is to build the compactification of a space by taking all \emph{maximal} bifilters. Note that McCallion does not require $\calF$ and $\calP$ to be filters, but rather arbitrary non-empty subsets. 

\paragraph{18-11-2023.} It's the weekend, but I'm porting over some Overleaf sections to this document. By \cref{theorem:strongly causal via Alexandrov topology} we know that a spacetime is strongly causal if and only if the chronological diamonds form a basis for the manifold topology. This is clearly a stronger statement than saying that the convex opens form a basis. What is the localic analogue of this? Namely, this theorem can be interpreted as saying that convex opens form a basis if and only if the IPs and IFs together form a basis?  Given an ordered locale, can we make a new locale out of intersection $F\wedge P$ of IFs and IPs?

\paragraph{24-11-2023.} Some good bits on the heuristic motivation of locales is in \emph{Notes on point-free topology}, Jorge Picado and Aleš Pultr.

\paragraph{13-12-2023.} Any strongly causal locale can be seen as a biframe. Now there is a literature of biframe compactifications that we can use. I'm trying to understand this now. 
On the way, we found that $\Up$ is a monad iff there is an adjunction $\Up \dashv \eta_\triangleup^{-1}$.

When is the biframe of a strongly causal locale regular, as a biframe? When does it admit a biframe compactification? In particular, does every spacetime admit a biframe compactification? Note spacetimes are regular as topological spaces. Are they biframe regular? Wouldn't that imply $T_2$-orderedness? And we know not every spacetime is even $T_0$-ordered. So that is a bit discouraging.

\paragraph{15-12-2023.} I've been thinking our localic approach is a bit pointless for the causal boundaries, since there exists work of e.g. Nachbin on compactification of ordered spaces already. So why do it localically? For spacetimes we should compare the two approaches.

\section{Chapter ideas and pointers to the literature}\label{section:literature draft}
Here I'll elaborate on some thoughts, also serving as a pointer to some literature that may be interesting, or that we will need to cite in the thesis. It's also a good opportunity to close a lot of tabs. Items will be added chronologically.
\begin{enumerate}[label = (\arabic*).]
	\item The article \cite{ling2020AspectsCausalTheory} has a nice appendix, and general results, showcasing the difference between causality in $C^0$ and smooth spacetimes. This is a nice reference to give when discussing the definition of the open cone condition. Particularly, their Proposition~A.1 discusses the \emph{push-up property} (see also Definition~4.2). Their push-up property says  $I^+\circ J^+ = I^+$. For the open cone condition, we are rather interested in the composition $J^+\circ I^+$. Is there a difference, or are these in some sense dual?
	
	The remark below Proposition~A.2 is exactly what we want to know though: there are $C^0$ spacetimes that do not satisfy $(J^+(p))^\circ = I^+(p)$. Hence such spacetimes fail the open cone condition (right?).
	
	\item The paper \cite{budic1974CausalBoundariesGeneral} has some ideas on characterising causal continuity and constructing causal completions by focussing on what they call ``set causality.'' (A related paper is \cite{hawking1974CausallyContinuousSpacetimes}.) They have some ideas on \emph{common future} and \emph{common past} that we can try to adopt to locales. A first guess would be to define the common future of $U$ as
	\[
	C^+U:= \Up\bigwedge\{\Up W:\varnothing\neq W\sqleq U\}.
	\]
	We need to prove some properties of this thing. (Unfortunately, the notation that seems common in the literature is to use $\up$ for $C^+$.) I don't see how to avoid the infinite meet operation here. 
	
	Using the common future/past, in Section~2.1 they define new causality and chronology relations on the set of future and past sets of the spacetime. Let's try to adopt that here. Let $P,Q\in \Opens X$ be past sets. Say $Q\chron P$ if and only if $P\wedge C^+Q\neq\varnothing$. If $X$ is parallel ordered, this will hold if and only if $\Down P \wedge \bigwedge_{W\sqleq Q}\Up W = \bigwedge_{W\sqleq Q}\Down P\wedge \Up W \neq\varnothing$. Can we unpack this further?
	
	In Definition~3.1 they define \emph{causally continuous} as meaning $I^+(x)\chron I^+(y)$ iff $x\chron y$ iff $I^-(x)\chron I^-(y)$ and $I^\pm$ being injective on points. The first condition is apparently equivalent to $C^+ I^-(x) = I^+(x)$ and $C^-I^+(x) = I^-(x)$. Such interactions between $C^\pm$ and the localic cones we can easily state in a locale, but the question is if we really need to evaluate these equations on points, or if open regions suffice. 
	
	\item Given a well-defined notion of the common future/past, $C^\pm$, can we use this to give an alternative definition of diamonds? Namely we would expect something like $U^\diamond = C^+C^- U \wedge C^-C^+ U$. Update: in the example of $\mathbb{R}^2$ with $(x,y)\leq (a,b)$ iff $x=a$ and $y\leq b$ is a counterexample to this. Namely $C^\pm U$ will always be empty, while $U^\diamond$ won't be.
	
	\item We should write a solid motivation to study locales, even without mentioning tensor topology. Probably \cite{johnstone1983PointPointlessTopology} would be the best to get a concise answer to this question. We should also look further into the literature of mereology, especially in relation to quantum mechanics. It would also be fun to mention some critiques of the mereological approach, as e.g. in \cite{russell2008StructureOfGunk}, especially their theorem on page~257. It will be good to start on this anyway, since it will help with introductions to talks, and the LFCS lab lunch. Just so I can close a bunch of tabs:
	\begin{enumerate}
		\item \cite{arntzenius2003QuantumMechanicsPointless} discusses mereology in relation to quantum mechanics. By the same author: \cite{arntzenius2011GunkTopologyMeasure}, seemingly an overview article;
		\item \cite{forrest1996HowInnocentMereology} is probably a further critique of mereology. By the same author, which we've cited before: \cite{forrest1996OntologyTopologyTheory};
	\end{enumerate}
	\item I should include in the introduction of the thesis an overview of how spacetime structure is recovered from the causal structure. 
\end{enumerate}

\section{Possible applications}
\begin{enumerate}[label = (\arabic*).]
	\item Through a suggestion of Tariq Elahi: Distance-bounding protocols. 
	\item Of course, the big one would be to study quantum teleportation, and similar such effects, using a suitable adoption of our framework to tensor topology, and hence categorical quantum mechanics. 
	\item Apply our ordered locales to study causality theory, in the sense of spacetimes. We are doing this now with Prakash.
	\item Apparently measure theory has a natural interpretation in the language of locales. How does that mix with our framework?
	\item There have been some papers studying causality/contextuality using sheaves. Of course, if you say locale, then you have to say sheaves. Does our framework have something to say there?
\end{enumerate}
}

\paragraph{Preface.} (\todo{I always imagined writing a really sappy preface. But lately I haven't been feeling that way any more. It has been a privilege being allowed to work on this project, and being allowed to take it into the direction that it has. Having never learned any lattice theory during my education (transitioning from a physics undergraduate to a mathematics postgraduate, somehow this got lost), it was a fun time learning about locales (and even just basic lattice theory). Similarly, I had done a course on the mathematical foundations of GR by Klaas Landsman. But, somehow, I am still left feeling I'm not particularly an expert in either.})




==> sections/preorders.tex <==
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{Preordered sets}
In this section we introduce the mathematical bedrock of this thesis: the notion of a \emph{preorder}. (\todo{The various properties of relations that might be suitable for a notion of causality are discussed in-depth in \cite{dribus2017DiscreteCausalTheory}.})

Preorders are most typically defined within the framework of sets and relations. Recall that a \emph{relation} $R$ between sets $X$ and $Y$ is (defined by) a subset $R\subseteq X\times Y$ of their cartesian product. Those pairs $(x,y)$ in $X\times Y$ that are contained in $R$ are said to be \emph{related} by $R$. As is common, we write $xRy$ whenever $(x,y)\in R$. A relation \emph{on} $X$ is just a relation from $X$ to itself. A preorder on $X$ is just a special type of relation on $X$:


\begin{definition}\label{definition:preorders}
	A \emph{preorder} (or \emph{preordered set}) is a set $P$, equipped with a relation $\leq$, satisfying the following two axioms:
	\begin{enumerate}[label=(\roman*)]
		\item $x\leq x$ for all $x\in P$; \hfill(\emph{reflexivity})
		\item if $x\leq y$ and $y\leq z$, then $x\leq z$. \hfill (\emph{transitivity})
	\end{enumerate}
	A \emph{partial order} (or \emph{poset}) is a preordered set $P$ satisfying additionally:
	\begin{enumerate}[label=(\roman*)]\setcounter{enumi}{2}
		\item $x\leq y$ and $y\leq x$ implies $x=y$. \hfill(\emph{anti-symmetry})
	\end{enumerate}
\end{definition}

\begin{remarknumbered}\label{remark:preorders are monads}
	A preorder is nothing but a \emph{monad} [\todo{ref}] in the 2-category $\Rel$. Indeed, a monad is a relation $R\colon P\to P$, and the existence of the unit and multiplication of the monad correspond precisely to the reflexivity and transitivity conditions of \cref{definition:preorders}. Such insights are exploited in the framework of \emph{Monoidal Topology}~\cite{hofmann2014MonoidalTopologyCategorical}. In \cref{proposition:properties of cones} we see another way to interpret order via monads.
\end{remarknumbered}

\begin{definition}\label{definition:monotone function between preorders}
	A function $g\colon P\to Q$ between preordered sets is called \emph{monotone} if $x\leq y$ implies $g(x)\leq g(y)$. We denote by $\Ord$ the category of preordered sets and monotone functions.
\end{definition}

Most of this thesis is dedicated to studying objects that are equipped with \emph{two} orders: an `intrinsic' partial order, describing a type of topology; and an `auxiliary' preorder, capturing what we generically call ``causality.'' The first one, usually denoted $\sqleq$, will be thought of as an abstract \emph{inclusion} relation. Hence we interpret $x\sqleq y$ as ``$x$ is contained in $y$,'' or ``$y$ contains $x$,'' and so forth. On the other hand, the preorder relation $\leq$ (and later also~$\Leq$) will be interpreted as encoding some type of causal information. Hence, whenever $x\leq y$, we say that $y$ is in the \emph{future} of $x$, and similarly that $x$ is in the \emph{past} of~$y$. The intrinsic order $\sqleq$ will often play a more subdued role in our notation.



A central theme of this thesis is the interplay between order and regions. In a preordered set this can be studied using the following concepts.

\begin{definition}\label{definition:cones}
	For a preordered set $(P,\leq)$, we define the \emph{up cone} and \emph{down cone} of a subset $A\subseteq P$, respectively, as:
	\[
	\up A:=\{x\in P:\exists a\in A: a\leq x\},
	\quad\text{and}\quad
	\down A:=\{y\in P:\exists a\in A: y\leq a \}.
	\]
	For singletons, we sometimes write $\up x:= \up\{x\}$ and $\down y := \down\{y\}$. With this notation, we can alternatively express the future and past cones as $\up A = \bigcup_{x\in A}\up x$ and $\down A= \bigcup_{y\in A}\down y$.
\end{definition}

\begin{remark}
	In the literature, the sets $\up A$ and $\down A$ are also typically called the \emph{upset} and \emph{downset} of $A$, respectively. Later, to further distinguish between the intrinsic and auxiliary orders, we will often also call $\up A$ and $\down A$ the \emph{future} and \emph{past cones} of $A$. The phrase ``cone'' comes from the notion of \emph{light cone} in relativity theory, which we discuss in-depth in \cref{section:causal relations of spacetime}.
\end{remark}

The up and down cones enjoy several nice properties.

\begin{lemma}\label{proposition:properties of cones}\label{lemma:properties of cones}
	If $(P,\leq)$ is a preordered set, then for any subsets $A,B\subseteq P$:
	\begin{enumerate}[label=(\alph*)]
		\item $\up A\subseteq \up B$ and $\down A\subseteq \down B$ whenever $A\subseteq B$;
		\item $A\subseteq \up A$ and $A\subseteq \down A$;
		\item $\up\up A\subseteq \up A$ and $\down\down A\subseteq \down A$.
	\end{enumerate}
	Further, for any family $(A_i)_{i\in I}$ of subsets of $P$:
	\begin{enumerate}[label=(\alph*)]\setcounter{enumi}{3}
		\item $\bigcup_{i\in I}\up A_i = \up\left(\bigcup_{i\in I}A_i\right)$ and $\bigcup_{i\in I}\down A_i = \down\left(\bigcup_{i\in I}A_i\right)$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	The first property follows by construction. The second and third follow by reflexivity and transitivity, respectively. For the final property, note first that $\up \varnothing = \varnothing = \down \varnothing$, so we may assume the index $I$ is non-empty. In that case, for every $j\in I$ we get $A_j\subseteq \bigcup_{i\in I}A_i$, so property~(a) already implies $\bigcup_{i\in I}\up A_i\subseteq \up\left(\bigcup_{i\in I} A_i\right)$. For the converse, pick $x\in \up\left(\bigcup_{i\in I}A_i\right)$. Then we can find $j\in I$ and $a\in A_j$ such that $a\leq x$. But this just means $x\in \up A_j$, and hence $x\in \bigcup_{i\in I}\up A_i$. The argument for the down cones is analogous.
\end{proof}

\begin{remark}
	In other words, we get join-preserving monads $\up(-)\colon\Powerset(P)\to \Powerset(P)$ and $\down(-)\colon \Powerset(P)\to\Powerset(P)$ on the powerset of $P$. Either one of these monads carry all the information of $\leq$, since:
	\[
	x\leq y
	\quad\text{if and only if}\quad
	x\in \down \{y\}
	\quad\text{if and only if}\quad
	y\in\up \{x\}.
	\]
	Note also that properties~(b) and~(c) of course combine to give strict equalities $\up \up A = \up A$ and $\down \down A=\down A$.
\end{remark}

A map of locales $f\colon X\to Y$ [\todo{ref}] is only defined in terms of its \emph{preimage} map $f^{-1}$, rather than something that takes the ``elements'' of $X$ to $Y$. The \cref{definition:monotone function between preorders} of monotonicity therefore does not readily adopt to this setting. For our purposes, the following lemma provides a suitable region-based alternative. 

\begin{lemma}\label{lemma:monotonicity in terms of cones}
	The following conditions for a function $g\colon P\to Q$ between preordered sets are equivalent:
	\begin{enumerate}[label=(\alph*)]
		\item $g$ is monotone (\cref{definition:monotone function between preorders});
		\item $\up g^{-1}(A)\subseteq g^{-1}(\up A)$ for all $A\subseteq Q$;
		\item $\down g^{-1}(A)\subseteq g^{-1}(\down A)$ for all $A\subseteq Q$.
	\end{enumerate}
\end{lemma}
\begin{proof}
	First we show that (a) implies (b). For that, take an element $y\in \up g^{-1}(A)$, meaning that there exists $x\in g^{-1}(A)$ with $x\leq y$. Monotonicity of $g$ implies $g(x)\leq g(y)$. But $g(x)\in A$, and hence $g(y)\in \up A$. Or, in other words: $y\in g^{-1}(\up A)$.
	
	For the converse, suppose that $x\leq y$ in $P$. This translates equivalently to $y\in \up \{ x\}$; moreover note that $x\in g^{-1}(\{g(x)\})$. Hence (b) implies:
	\[
	y\in \up \{x\}\subseteq \up g^{-1}(\{g(x)\})\subseteq g^{-1}(\up\{g(x)\}).
	\]
	But this just means $g(y)\in \up\{g(x)\}$, that is: $g(x)\leq g(y)$. The equivalence between (a) and (c) is proved dually.
\end{proof}

Another characterisation that is more abstract is as follows.
\begin{lemma}
	A function $g\colon P\to Q$ between preordered sets is monotone if and only if there is an arrow making the following square commute:
	\[
	% https://q.uiver.app/#q=WzAsNCxbMCwwLCJcXGdyYXBoKFxcbGVxX1ApIl0sWzEsMCwiXFxncmFwaChcXGxlcV9RKSJdLFswLDEsIlBcXHRpbWVzIFAiXSxbMSwxLCJRXFx0aW1lcyBRLiJdLFswLDIsIiIsMCx7InN0eWxlIjp7InRhaWwiOnsibmFtZSI6Imhvb2siLCJzaWRlIjoidG9wIn19fV0sWzEsMywiIiwwLHsic3R5bGUiOnsidGFpbCI6eyJuYW1lIjoiaG9vayIsInNpZGUiOiJ0b3AifX19XSxbMCwxLCJcXGV4aXN0cyBcXG92ZXJsaW5le2d9IiwwLHsic3R5bGUiOnsiYm9keSI6eyJuYW1lIjoiZGFzaGVkIn19fV0sWzIsMywiZ1xcdGltZXMgZyIsMl1d
	\begin{tikzcd}[ampersand replacement=\&]
		{\graph(\leq_P)} \& {\graph(\leq_Q)} \\
		{P\times P} \& {Q\times Q.}
		\arrow[hook, from=1-1, to=2-1]
		\arrow[hook, from=1-2, to=2-2]
		\arrow["{\exists \overline{g}}", dashed, from=1-1, to=1-2]
		\arrow["{g\times g}"', from=2-1, to=2-2]
	\end{tikzcd}
	\]
\end{lemma}
\begin{proof}
	(\todo{Prove. Relevant for internal preorders.})
\end{proof}

\begin{remark}
	Note that since the inclusion $\graph(\leq_Q)\hookrightarrow Q\times Q$ is a monomorphism, the arrow $\overline{g}$, if it exists, is the unique such that makes the diagram commute.
\end{remark}

==> sections/strict-adjunction.tex <==
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\section{Another adjunction: localic chronology}
In this section we briefly describe a frame-theoretic version of the notion of a \emph{causal sites} from \cite{christensen2005CausalSitesQuantum}. We prove that there is an adjunction between a certain category of \emph{strictly} and \emph{strictly} ordered locales. Historically, the work in this section was developed before the theory of ordered locales. Since ordered spaces are more prevalent than \emph{strictly} ordered spaces, the newer framework is preferred. 

The idea is roughly to define a point-free analogue $\Chron$ of the chronology relation~$\chron$ of a spacetime. The appropriate mathematical framework of the point-wise side is that of strictly ordered spaces.

\begin{definition}
	A \emph{strictly partially ordered space} (or \emph{spospace} for short) is a pair $(S,\chron)$ consisting of a topological space $S$ together with a strict partial order on the underlying set of $S$. Recall this means $\chron$ is a irreflexive and transitive relation:
		\begin{enumerate}[label = (\roman*)]
			\item $x\chron y\chron z$ implies $x\chron z$;
			\item $x\not\chron x$ for all $x$.
		\end{enumerate}
	
	A morphism of spospaces $g\colon (S,\chron)\to (T,\chron)$ consists of a continuous function $g\colon S\to T$ such that if $x\chron y$ then $g(x)\chron g(y)$. We refer to these morphisms also as \emph{monotone}. The category spospaces and monotone continuous functions is denoted by~$\SpoTop$.
\end{definition}

Compare this to the definition of \emph{chronological sets} from \cite{harris1997UniversalityFutureChronological}.


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{Chronological semilattices}
\begin{definition}
	A \emph{pre-chronological semilattice} is a meet-semilattice $L$ with bottom element $\bot\in L$, together with a relation $\Chron$ on $L$ that is transitive and irreflexive on non-empty elements:
		\begin{enumerate}[label =(\roman*)]
			\item for all $x,y,z\in L\setminus\{\bot\}$, if $x\Chron y\Chron z$ then $x\Chron z$;
			\item for all $x\in L\setminus \{\bot\}$ we have $x\not\Chron x$.
		\end{enumerate}
\end{definition}

The following definition imposes a relation between the semilattice and chronological structures.

\begin{definition}
	A \emph{chronological semilattice} is a pre-chronological semilattice $(L,\Chron)$ satisfying the following axioms:
		\begin{enumerate}[leftmargin=3\parindent]
			\item[($\wedge^-$)] if $x\Chron z$ then $x\wedge y\Chron z$;
			\item[($\wedge^+$)] if $x\Chron z$ then $x\Chron y\wedge z$;
			\item[($\Chron$$\bot$)] for all $x\in L$ we have $\bot\Chron x\Chron \bot$;
			\item[($\Chron$D)] if $x\Chron y$ then $x\wedge y = \bot$. 
		\end{enumerate}
\end{definition}

These axioms are very similar to the axioms of \emph{causal sites} \cite{christensen2005CausalSitesQuantum}. Causal sites are essentially poset generalisations of chronological semilattices. They have two axioms of the form
	\begin{enumerate}[leftmargin=3\parindent]
		\item[(CS5)] if $x\sqleq y$ and $y\Chron z$, then $x\Chron z$;
		\item[(CS6)] if $x\sqleq y$ and $z\Chron y$, then $z\Chron x$.
	\end{enumerate}

\begin{lemma}
	In a pre-chronological semilattice:
		\begin{enumerate}[label = (\alph*)]
			\item axiom (CS5) holds if and only if axiom~\eqref{axiom:wedge-} holds;
			\item axiom (CS6) holds if and only if axiom~\eqref{axiom:wedge+} holds.
		\end{enumerate}
\end{lemma}

\begin{example}
	The motivating example comes from strictly ordered sets. For any set $S$ with a strict partial order $<$, the powerset $\Powerset(S)$ is a chronological semilattice where the order is defined as:
		\[
			A\Chron B
			\qquad\text{if and only if}\qquad
			\forall a\in A\forall b\in B\colon a<b.
		\]
\end{example}


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{Chronological locales}
We are now ready to state the definition of chronological locales.
\begin{definition}
	A \emph{chronological locale} $(X,\Chron)$ is a locale $X$ whose frame of opens $\Opens X$ is equipped with a chronological semilattice structure $\Chron$, such that the following two axioms hold:
		\begin{enumerate}[leftmargin=3\parindent]
			\item[($\vee^-$)] $\bigvee_{i\in I} U_i\Chron V$ if and only if $\forall i\in I\colon U_i\Chron V$;
			\item[($\vee^+$)] $U\Chron \bigvee_{i\in I} V_i$ if and only if $\forall i\in I\colon U\Chron V_i$.
		\end{enumerate}
\end{definition}

\begin{remark}
	The axioms ($\vee^\pm$) are infinitary versions of axioms for a causal site. 
\end{remark}

The definition of monotonicity is very similar to the \cref{definition:monotone map of ordered locales} of monotone maps between ordered locales.
\begin{definition}
	A \emph{morphism of chronological locales} $f\colon (X,\Chron)\to (Y,\Chron)$ is a map of locales $f\colon X\to Y$ such that:
		\[
		\begin{tikzcd}[every label/.append style = {font = \normalsize},column sep=0.3cm, row sep=0.35cm]
			{U} & {U'} \\
			{V} & {\highlighttikzcd{\exists V'}}
			\arrow["R_f"{anchor=center}, draw=none, from=2-1, to=1-1]
			\arrow["R_f"{anchor=center}, draw=none, from=2-2, to=1-2]
			\arrow["{}"{description}, "\Chron"{anchor=center}, draw=none, from=1-1, to=1-2]
			\arrow["{}"{description}, "\Chron"{anchor=center}, draw=none, from=2-1, to=2-2]
		\end{tikzcd}
		\qquad\text{and}\qquad 
		\begin{tikzcd}[every label/.append style = {font = \normalsize},column sep=0.3cm, row sep=0.35cm]
			{U} & {U'} \\
			\highlighttikzcd{\exists V} & {V'.}
			\arrow["R_f"{anchor=center}, draw=none, from=2-1, to=1-1]
			\arrow["R_f"{anchor=center}, draw=none, from=2-2, to=1-2]
			\arrow["{}"{description}, "\Chron"{anchor=center}, draw=none, from=1-1, to=1-2]
			\arrow["{}"{description}, "\Chron"{anchor=center}, draw=none, from=2-1, to=2-2]
		\end{tikzcd}		
		\]
\end{definition}

\begin{proposition}
	There is a category $\ChronLoc$ of chronological locales and monotone maps of locales.
\end{proposition}

==> symbols/TikzEdt_files/causl.tex <==
\usetikzlibrary{arrows}
\begin{tikzpicture}
\node {$\prec$};
\draw[line cap=round] (0.1,0.09475) .. controls (0.125,0) and (0.125,0) .. (0.1,-0.09475);
\end{tikzpicture}


==> tikz/inkscape-export/drafts/fig <==

\definecolor{cffebdc}{RGB}{255,235,220}
\definecolor{cffffdc}{RGB}{255,255,220}
\definecolor{c644700}{RGB}{100,71,0}
\definecolor{c640000}{RGB}{100,0,0}
\definecolor{cefffff}{RGB}{239,255,255}
\definecolor{c001764}{RGB}{0,23,100}


\def \globalscale {1.000000}
\begin{tikzpicture}[y=1pt, x=1pt, yscale=\globalscale,xscale=\globalscale, every node/.append style={scale=\globalscale}, inner sep=0pt, outer sep=0pt]
  \begin{scope}[shift={(-271.503, 73.658)}]
    \path[fill=cffebdc,line width=1.0pt] (399.75, -48.128) -- (399.75, 22.738) 
  -- (340.222, 22.738) -- (310.457, -16.948) -- (279.472, -14.922) -- (272.19, 
  -5.229) -- (272.19, -48.128) -- (300.536, -48.128) -- (343.056, 8.564) -- 
  (385.576, -48.128) -- cycle;



    \path[fill=black,line width=1.0pt] (343.272, 8.565) ellipse (1.417pt and 
  1.417pt);



    \path[fill=cffffdc,line width=1.0pt] (340.222, 22.738) -- (272.19, 22.738) 
  -- (272.19, -5.229) -- (279.472, -14.922) -- (310.457, -16.948) -- cycle;



    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (343.056, 8.565) -- (300.537, 
  -48.128);



    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (340.395, 22.969) -- (310.458, 
  -16.947);



    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (343.056, 8.565) -- (385.576, 
  -48.128);



    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (272.225, -5.348) -- (282.044, 
  -18.439);



    \node[text=black,line cap=butt,line join=miter,line width=1.001pt,miter 
  limit=4.0,anchor=south west] (text3) at (347.327, 8.565){$x$};



    \path[draw=black,fill=cffffdc,line cap=butt,line join=miter,line 
  width=1.0pt,miter limit=4.0] (297.702, -11.278).. controls (292.061, -10.71) 
  and (283.674, -6.455) .. (280.694, -11.278).. controls (278.111, -15.459) and 
  (282.969, -22.123) .. (287.291, -24.463).. controls (292.035, -27.032) and 
  (298.654, -25.235) .. (303.371, -22.616).. controls (306.636, -20.804) and 
  (311.62, -17.356) .. (310.343, -13.847).. controls (308.871, -9.807) and 
  (301.98, -11.708) .. (297.702, -11.278) -- cycle;



    \node[text=c644700,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,anchor=south west] (text5) at (289.69, -20.203){$F$};



    \node[text=c644700,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,anchor=south west] (text7) at (288.57, 4.359){$\Up F$};



    \node[text=c640000,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,anchor=south west] (text12) at (366.116, 
  -11.275){$\eta^\triup_\ast(P_x)$};



  \end{scope}
%  \begin{scope}[]
%    \path[draw=black,fill=cffebdc,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 66.388) circle (4.496pt);
%
%
%
%    \path[draw=black,fill=cefffff,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 55.537) circle (4.496pt);
%
%
%
%    \path[draw=black,fill=cffffdc,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 44.199) circle (4.496pt);
%
%
%
%    \node[text=c001764,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text6-4-3) at (-59.214, 53.865){$text$};
%
%
%
%    \node[text=c001764,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text6-4-3-2) at (-59.214, 64.403){$text$};
%
%
%
%    \node[text=c644700,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text11-9-5-1-4-5) at (-59.214, 43.326){$text$};
%
%
%
%    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
%  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (-33.328, 68.049) -- (-33.328, 
%  39.703);
%
%
%
%  \end{scope}

\end{tikzpicture}


==> tikz/inkscape-export/drafts/fig-06 <==

\definecolor{cefffff}{RGB}{239,255,255}
\definecolor{cffebdc}{RGB}{255,235,220}
\definecolor{c004100}{RGB}{0,65,0}
\definecolor{cffb809}{RGB}{255,184,9}
\definecolor{c640000}{RGB}{100,0,0}
\definecolor{c001764}{RGB}{0,23,100}
\definecolor{cffffdc}{RGB}{255,255,220}
\definecolor{c644700}{RGB}{100,71,0}


\def \globalscale {1.000000}
\begin{tikzpicture}[y=1pt, x=1pt, yscale=\globalscale,xscale=\globalscale, every node/.append style={scale=\globalscale}, inner sep=0pt, outer sep=0pt]
  \begin{scope}[shift={(-271.503, 73.658)}]
    \path[fill=cefffff,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0] (335.54, 1.906) -- (398.884, 65.202) -- (272.197, 65.251) -- cycle;



    \path[fill=cefffff,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0] (335.54, 1.906) -- (272.197, -61.439) -- (398.884, -61.439) -- 
  cycle;



    \path[fill=cffebdc,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0] (335.54, 1.89) -- (398.884, 65.202) -- (398.884, -61.422) -- cycle;



    \path[fill=cffebdc,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0] (272.197, 65.202) -- (335.54, 1.89) -- (272.197, -61.422) -- cycle;



    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (335.54, 1.89) -- (398.884, 65.202);



    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (272.197, 65.202) -- (335.54, 1.89)
   -- (272.197, -61.422);



    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (335.54, 1.89) -- (398.884, 
  -61.422);



    \node[text=black,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,scale=1.0,anchor=south west] (text4) at (341.419, -1.373){$x$};



    \node[text=black,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,scale=1.0,anchor=south west] (text4-4) at (347.91, 48.575){$y$};



    \node[text=black,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,scale=1.0,anchor=south west] (text4-4-5) at (284.794, 31.408){$y'$};



    \node[text=black,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,scale=1.0,anchor=south west] (text4-0) at (294.123, -45.789){$z$};


	\begin{scope}[decoration={
	markings,% switch on markings
	mark=between positions .45 and .95 step 30pt with {\arrow[line width = .75pt]{>}}}
	]
    \path[postaction = {decorate},draw=c004100,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0] (299.475, -61.422).. controls (299.475, -61.422) and (299.29, 
  -56.475) .. (304.924, -43.538).. controls (307.073, -38.605) and (319.973, 
  -23.135) .. (328.883, -11.278).. controls (334.81, -3.391) and (335.54, 1.89) 
  .. (335.54, 1.89);



    \path[postaction = {decorate},draw=c004100,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0] (335.54, 1.89).. controls (335.54, 1.89) and (337.248, 14.572) .. 
  (338.291, 20.883).. controls (339.883, 30.505) and (343.131, 38.994) .. 
  (343.643, 49.647).. controls (343.986, 56.76) and (339.763, 65.202) .. 
  (339.763, 65.202);
	\end{scope}


	\begin{scope}[decoration={snake, amplitude = 1pt, segment length = 6pt}]
\path[decorate, ->,draw=cffb809,line cap=butt,line join=miter,line width=1.0pt,miter 
limit=4.0] (335.54, 1.89) -- (297.534, 39.877);
\end{scope}


    \path[fill=black,line width=1.0pt] (335.489, 1.89) ellipse (2.111pt and 
  2.11pt);



    \path[fill=black,line width=1.0pt] (304.924, -43.492) ellipse (2.111pt and 
  2.11pt);



    \path[fill=black,line width=1.0pt] (297.363, 39.877) ellipse (2.111pt and 
  2.11pt);



    \path[fill=black,line width=1.0pt] (343.643, 49.778) ellipse (2.111pt and 
  2.11pt);



    \node[text=c640000,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,anchor=south west,align=center,execute at begin node=\setlength{\baselineskip}{0pt}] (text11) at (270, -10){spacelike\\separated};



    \node[text=c001764,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,anchor=south west,align =center,execute at begin node=\setlength{\baselineskip}{0pt}] (text12) at (325, -50){timelike\\separated};



  \end{scope}
%  \begin{scope}[]
%    \path[draw=black,fill=cffebdc,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 66.388) circle (4.496pt);
%
%
%
%    \path[draw=black,fill=cefffff,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 55.537) circle (4.496pt);
%
%
%
%    \path[draw=black,fill=cffffdc,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 44.199) circle (4.496pt);
%
%
%
%    \node[text=c001764,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text6-4-3) at (-59.214, 53.865){$text$};
%
%
%
%    \node[text=c001764,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text6-4-3-2) at (-59.214, 64.403){$text$};
%
%
%
%    \node[text=c644700,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text11-9-5-1-4-5) at (-59.214, 43.326){$text$};
%
%
%
%    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
%  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (-33.328, 68.049) -- (-33.328, 
%  39.703);
%
%
%
%  \end{scope}

\end{tikzpicture}


==> tikz/inkscape-export/drafts/fig-working <==

\definecolor{cffffdc}{RGB}{255,255,220}
\definecolor{c001764}{RGB}{0,23,100}
\definecolor{cefffff}{RGB}{239,255,255}
\definecolor{c0d6400}{RGB}{13,100,0}
\definecolor{ce0ffdc}{RGB}{224,255,220}
\definecolor{c640000}{RGB}{100,0,0}
\definecolor{cffebdc}{RGB}{255,235,220}
\definecolor{c644700}{RGB}{100,71,0}


\def \globalscale {1.000000}
\begin{tikzpicture}[y=1pt, x=1pt, yscale=\globalscale,xscale=\globalscale, every node/.append style={scale=\globalscale}, inner sep=0pt, outer sep=0pt]
  \node[text=black,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,anchor=south west] (text2) at (82.47, 8.595){$U$};



  \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (80.058, 14.191) -- (109.978, 
  96.395);



  \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (48.876, 11.356) -- (17.816, 
  96.395);


\begin{scope}[blend group = multiply]
  \path[draw=black,fill=cffffdc,line cap=butt,line join=miter,line 
  width=1.0pt,miter limit=4.0] (50.455, 17.423).. controls (48.802, 16.145) and 
  (47.88, 13.193) .. (48.876, 11.356).. controls (50.302, 8.73) and (54.707, 
  9.856) .. (57.38, 8.521).. controls (59.7, 7.364) and (61.188, 4.168) .. 
  (63.78, 4.104).. controls (70.161, 3.946) and (77.657, 8.276) .. (80.058, 
  14.191).. controls (81.523, 17.801) and (79.978, 22.775) .. (77.223, 25.529)..
   controls (74.468, 28.284) and (69.169, 30.459) .. (65.884, 28.364).. controls
   (62.753, 26.367) and (66.643, 19.788) .. (63.78, 17.423).. controls (60.355, 
  14.595) and (53.969, 20.14) .. (50.455, 17.423) -- cycle;



  \path[draw=c001764,fill=cefffff,line cap=butt,line join=miter,line 
  width=0.7pt,miter limit=4.0,dash pattern=on 5.6pt off 0.7pt] (31.869, 
  65.214).. controls (25.08, 70.422) and (23.505, 84.196) .. (29.034, 90.726).. 
  controls (34.695, 97.412) and (46.519, 91.933) .. (55.276, 92.174).. controls 
  (65.422, 92.452) and (82.864, 101.904) .. (85.727, 92.166).. controls (87.946,
   84.618) and (72.484, 83.67) .. (65.884, 79.388).. controls (59.897, 75.502) 
  and (54.629, 70.219) .. (47.962, 67.67).. controls (42.893, 65.732) and 
  (36.174, 61.912) .. (31.869, 65.214) -- cycle;



  \path[draw=c001764,fill=cefffff,line cap=butt,line join=miter,line 
  width=0.7pt,miter limit=4.0,dash pattern=on 5.6pt off 0.7pt] (40.056, 
  37.889).. controls (38.173, 32.935) and (44.09, 26.516) .. (49.111, 24.821).. 
  controls (61.954, 20.486) and (84.539, 24.211) .. (87.789, 37.37).. controls 
  (88.999, 42.268) and (82.115, 46.975) .. (77.223, 48.206).. controls (71.114, 
  49.745) and (65.263, 44.226) .. (59.194, 42.537).. controls (52.869, 40.777) 
  and (42.388, 44.026) .. (40.056, 37.889) -- cycle;



  \path[draw=c0d6400,fill=ce0ffdc,line cap=butt,line join=miter,line 
  width=0.7pt,miter limit=4.0,dash pattern=on 5.6pt off 0.7pt] (66.645, 
  59.545).. controls (63.445, 59.977) and (59.846, 58.796) .. (57.38, 56.71).. 
  controls (54.154, 53.982) and (50.627, 49.456) .. (51.711, 45.372).. controls 
  (52.586, 42.079) and (56.81, 39.82) .. (60.215, 39.703).. controls (67.828, 
  39.44) and (79.883, 43.425) .. (80.058, 51.041).. controls (80.179, 56.333) 
  and (71.891, 58.837) .. (66.645, 59.545) -- cycle;



  \path[draw=c0d6400,fill=ce0ffdc,line cap=butt,line join=miter,line 
  width=0.7pt,miter limit=4.0,dash pattern=on 5.6pt off 0.7pt] (86.841, 
  90.437).. controls (80.743, 90.286) and (70.277, 93.789) .. (68.719, 87.892)..
   controls (66.741, 80.404) and (79.67, 75.804) .. (87.129, 73.718).. controls 
  (90.924, 72.657) and (95.728, 72.656) .. (98.878, 75.024).. controls (102.861,
   78.018) and (107.174, 84.574) .. (104.593, 88.837).. controls (101.517, 
  93.92) and (92.781, 90.585) .. (86.841, 90.437) -- cycle;



  \path[draw=c640000,fill=cffebdc,line cap=butt,line join=miter,line 
  width=0.7pt,miter limit=4.0,dash pattern=on 8.4pt off 0.7pt] (33.828, 
  65.503).. controls (38.449, 74.744) and (52.5, 77.008) .. (62.818, 76.469).. 
  controls (75.272, 75.819) and (99.488, 71.703) .. (96.244, 59.661).. controls 
  (93.242, 48.52) and (72.875, 64.595) .. (61.693, 61.75).. controls (53.054, 
  59.553) and (47.342, 44.393) .. (39.016, 47.577).. controls (33.205, 49.799) 
  and (31.045, 59.94) .. (33.828, 65.503) -- cycle;
\end{scope}


  \node[text=black,line cap=butt,line join=miter,line width=1.0pt,miter 
  limit=4.0,anchor=south west] (text7) at (105.188, 67.323){$\Up U$};



%  \begin{scope}[]
%    \path[draw=black,fill=cffebdc,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 66.388) circle (4.496pt);
%
%
%
%    \path[draw=black,fill=cefffff,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 55.537) circle (4.496pt);
%
%
%
%    \path[draw=black,fill=cffffdc,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 44.199) circle (4.496pt);
%
%
%
%    \path[draw=black,fill=ce0ffdc,line cap=butt,line join=miter,line 
%  width=1.0pt,miter limit=4.0] (-41.832, 32.86) circle (4.496pt);
%
%
%
%    \node[text=c001764,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text6-4-3) at (-59.214, 53.865){$text$};
%
%
%
%    \node[text=c640000,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text6-4-3-2) at (-59.214, 64.403){$text$};
%
%
%
%    \node[text=c644700,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text11-9-5-1-4-5) at (-59.214, 43.326){$text$};
%
%
%
%    \node[text=c0d6400,line cap=butt,line join=miter,line width=1.0pt,miter 
%  limit=4.0,anchor=south west] (text11-9-5-1-4-5-6) at (-59.214, 32.787){$text$};
%
%
%
%    \path[draw=black,line cap=butt,line join=miter,line width=0.5pt,miter 
%  limit=4.0,dash pattern=on 0.5pt off 2.0pt] (-33.328, 68.049) -- (-33.328, 
%  28.364);
%
%
%
%  \end{scope}

\end{tikzpicture}


==> tikz/inkscape-export/drafts/macros.tex <==
%general
\newcommand{\todo}[1]{{\color{Bittersweet}#1}}
\newcommand{\todobig}[1]{{\color{Bittersweet}#1}}

%general math
\newcommand{\comp}{\mathbin{\circ}}
\newcommand{\Opens}{\mathop{\mathcal{O}\mspace{-4mu}}}
\newcommand{\AOpens}{\mathop{\mathcal{OA}\mspace{-4mu}}}
\newcommand{\Powerset}{\mathop{\mathcal{P}\!}}
\newcommand{\Sl}{\mathop{\mathrm{S}\ell}\mspace{-1mu}}
\DeclareMathOperator{\graph}{graph}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\id}{id}
\newcommand{\pr}{\mathrm{pr}}
\newcommand{\sqleq}{\sqsubseteq} 
\newcommand{\sqgeq}{\sqsupseteq}
\DeclareMathOperator{\dom}{dom}
\newcommand{\op}{{\mathrm{op}}}
\DeclareMathOperator{\Ideals}{\mathfrak{I}}
\DeclareMathOperator{\ideal}{\mathfrak{i}}
\DeclareMathOperator{\RegIdeals}{\mathfrak{R}}
\DeclareMathOperator{\Filters}{\mathfrak{F}}
\DeclareMathOperator{\filter}{\mathfrak{f}}
\newcommand{\tensor}{\otimes}
\newcommand{\aleq}{\mathrel{\triangleleft}}
\DeclareMathOperator{\IP}{IP}
\DeclareMathOperator{\IF}{IF}
\newcommand{\hull}[1]{\widehat{#1}}
\DeclareMathOperator{\MSub}{\calM Sub}
\DeclareMathOperator*{\colim}{colim}
\newcommand{\disj}{\mathbin{\bowtie}}
\DeclareMathOperator{\OL}{OL}
\DeclareMathOperator{\Monads}{Monads}
\newcommand{\refines}{\Subset}
\newcommand{\Refines}{\subset}
\newcommand{\atomicbelow}{\lessdot}
\def\dashedboxtikz{\tikz\node[draw=black,thick,densely dashed] {\phantom{x}};}
\newcommand{\inlinedashedbox}[1]{\tikz[baseline]{\node[draw=black,thick,densely dashed,anchor=base] {\phantom{#1}};}}

% notation style
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\epsilon}{\varepsilon}

%shorthands
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\aqft}{\textsc{aqft}}
\newcommand{\aqfts}{\aqft s}

%ordered sets/locales
\newcommand{\Leq}{\mathrel{\trianglelefteqslant}}
\newcommand{\up}{\mathop{\uparrow}\!}
\newcommand{\down}{\mathop{\downarrow}\!}
\newcommand{\triup}{\text{\rotatebox[origin=c]{-90}{$\triangleleft$}}}
\newcommand{\tridown}{\text{\rotatebox[origin=c]{90}{$\triangleleft$}}}

%localic cones %https://tex.stackexchange.com/a/506063
\usepackage{trimclip}
\makeatletter
\newcommand{\tworightarrow}{\mathrel{\text{\two@rightarrow}}}
\newcommand{\two@rightarrow}{%
	\sbox0{$\m@th\rightarrow$}%
	\smash{\rlap{\kern0.1\wd0\clipbox{{.3\width} {-\height} 0pt {-\height}}{$\m@th\rightarrow$}}}%
	$\m@th\rightarrow$%
}
\makeatletter
\newcommand{\twoleftarrow}{\mathrel{\text{\two@leftarrow}}}
\newcommand{\two@leftarrow}{%
	\sbox0{$\m@th\leftarrow$}%
	\smash{\rlap{\kern0.1\wd0\clipbox{{-.1\width} {-\height} 3pt {-\height}}{$\m@th\leftarrow$}}}%
	$\m@th\leftarrow$%
}

\newcommand{\uup}{\mspace{3mu}\mathop{\rotatebox[y=.65\height]{90}{$\tworightarrow$}}\mspace{-1mu}}
\newcommand{\ddown}{\mspace{3mu}\mathop{\rotatebox[y=.65\height]{90}{$\twoleftarrow$}}\mspace{-1mu}}

\newcommand{\preUp}{\scalebox{1.2}[1.05]{\rotatebox[origin=c]{90}{$\rightarrowtriangle$}}}
\newcommand{\preDown}{\scalebox{1.2}[1.05]{\rotatebox[origin=c]{-90}{$\rightarrowtriangle$}}}

\newcommand{\Up}{\text{\preUp}}
\newcommand{\Down}{\text{\preDown}}
\newcommand{\Upsub}[1]{\Up_{\mspace{-3.5mu}#1}}
\newcommand{\Downsub}[1]{\Down_{\mspace{-1.5mu}#1}}
\newcommand{\Upi}{\Upsub{i}}
\newcommand{\Downi}{\Downsub{i}}


%Coverages
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\CovLeq}{\Cov_{\Leq}}
\newcommand{\Covcaus}{\mathrm{Caus}}
\newcommand{\Covchron}{\mathrm{Chron}}
\newcommand{\JLeq}{J_{\Leq}}
\newcommand{\Dcaus}{D_{\caus}}
\newcommand{\Dchron}{D_{\chron}}
\newcommand{\DCaus}{D_\Covcaus}
\newcommand{\DChron}{D_\Covchron}
\newcommand{\DLeq}{D_{\Leq}}

%list of categories
\newcommand{\cat}[1]{\mathbf{#1}}
\newcommand{\Set}{\cat{Set}}
\newcommand{\Top}{\cat{Top}}
%\newcommand{\Frame}{\cat{Frm}}
\newcommand{\Frm}{\cat{Frm}}
%\newcommand{\Locale}{\cat{Loc}}
\newcommand{\Loc}{\cat{Loc}}
\newcommand{\Preord}{\cat{Preord}}
\newcommand{\Poset}{\cat{Poset}}
\newcommand{\Ord}{\cat{Ord}}
\newcommand{\OrdLoc}{\cat{OrdLoc}}
\newcommand{\OrdTop}{\cat{OrdTop}}
\newcommand{\SpoTop}{\cat{SpoTop}}
\newcommand{\ChronLoc}{\cat{ChronLoc}}
\newcommand{\OC}{\mathrm{OC}}
\newcommand{\Rel}{\cat{Rel}}
\newcommand{\OrdC}{\mathrm{Ord}(\cat{C})}
\newcommand{\OrdD}{\mathrm{Ord}(\cat{D})}
\newcommand{\FBT}{\cat{P}}
\newcommand{\Diffeol}{\cat{Diffeol}}
\newcommand{\ord}{\mathrm{Ord}}
\newcommand{\Site}{\cat{Site}}

%functors
\DeclareMathOperator{\pt}{pt}
\DeclareMathOperator{\pf}{pf}
\DeclareMathOperator{\loc}{Loc}
\DeclareMathOperator{\Kleisli}{K\mspace{-1mu}\ell}
\DeclareMathOperator{\Sh}{Sh}

%causality relations
\newcommand{\ratherbelow}{\prec}
\newcommand{\completelybelow}{\prec\mspace{-3mu}\prec}
\newcommand{\caus}{\mathrel{\preccurlyeq}}
\newcommand{\causeq}{\mathrel{\preccurlyeq}}
%defines nice chronology relation as in the Kronheimer Penrose paper
\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
	<5> <6> <7> <8> <9> <10> gen * matha
	<10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
}{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}
\DeclareMathSymbol{\prechron}{3}{matha}{'316} 
\newcommand{\chron}{\mathrel{\prechron}}
\newcommand{\ileq}{\chron}

% old localic chronology relation:
%\makeatletter
%\newcommand{\Chronold}{\mspace{-.8mu}\mathrel{\text{\localic@chron}}}
%\newcommand{\localic@chron}{%
%	\sbox0{$\m@th\chron$}%
%	\smash{\rlap{\kern.7\wd0\clipbox{{0\width} {.245\height} 0pt {.24\height}}{$\m@th\vert$}}}%
%	$\m@th\chron$%
%}
%
%\makeatletter
%\newcommand{\Chron}{\mspace{-1mu}\mathrel{\scalebox{.95}[1.1]{\text{\localic@chronalt}}}}
%\newcommand{\localic@chronalt}{%
%	\sbox0{$\m@th\vartriangleleft$}%
%	\smash{\rlap{\kern.45\wd0\raisebox{.9pt}{{$\m@th\scalebox{.7}[.6]{$\triangleleft$}$}}}}%
%	$\m@th\vartriangleleft$%
%}

% hand-drawn chronology relation
\makeatletter
\newcommand*\chronltemp{\mathrel{\raisebox{0.4\depth}{$\vcenter{\hbox{\includegraphics[width=0.65em]{symbols/chronl.png}}}$}}}
\makeatother
\newcommand{\Chron}{\chronltemp}

==> tikz/inkscape-export/drafts/preamble.tex <==
% packages
\usepackage[british]{babel}

%typesetting: turn off for laptop
\usepackage{mlmodern} %"denser" letters
\usepackage[T1]{fontenc}



%math
\usepackage[leqno]{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{stmaryrd}
\usepackage[mathcal]{euscript}

%figures and colours
\usepackage{caption}
\captionsetup[wrapfigure]{font=footnotesize}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{epigraph}
\usepackage[dvipsnames]{xcolor}
\definecolor{LinkColor}{HTML}{617181}%{20, 60, 94}%{224, 102, 102}%{21,48,132}
\definecolor{CiteColor}{HTML}{84A59D}
\usepackage[colorlinks=true,linkcolor=LinkColor,citecolor=CiteColor%Cerulean
,urlcolor=BurntOrange]{hyperref}
\usepackage[capitalise,nameinlink,noabbrev]{cleveref}

%colourbox
\usepackage[most]{tcolorbox}
\definecolor{HighlightColor}{HTML}{DDFFCD}
\tcbset{on line, toprule=-2pt, bottomrule=-2pt,
	boxsep=2pt, left=0pt,right=0pt,top=0pt,bottom=0pt,
	colframe = white, colback=HighlightColor,  
	highlight math style={enhanced}
}
\newcommand{\highlighttikzcd}[1]{\tcbhighmath{#1}}
%\newcommand{\highlighttikzcd}[1]{\colorbox{HighlightColor}{$\displaystyle #1$}}

\usepackage{titlesec}
\titlespacing*{\section}
{0pt}{1ex}{1ex}  %<indent><top sep><bottom sep>


%https://tex.stackexchange.com/a/283066/100286
\makeatletter
\newcommand{\dummylabel}[2]{\def\@currentlabel{#2}\label{#1}}
\makeatother

%bibliography
\usepackage[backend=bibtex,style=alphabetic,defernumbers=true,doi=false,isbn=false,url=false,useprefix=true,sorting =nyt,backref=true,giveninits=true,maxnames=99,maxalphanames=99]{biblatex} %,maxnames=10,minnames=9,maxbibnames=99,maxalphanames=10,minalphanames=9,firstinits=true
\bibliography{bibliography.bib}
%\renewcommand*{\bibfont}{\footnotesize} %changes the bibliography font size
	%makes cite labels bold:
%	\DeclareFieldFormat{labelalpha}{\mkbibbold{#1}}
%	\DeclareFieldFormat{extraalpha}{\mkbibbold{\mknumalph{#1}}}
%	\AtBeginBibliography{
%		\DeclareFieldFormat{labelalpha}{#1}
%		\DeclareFieldFormat{extraalpha}{\mknumalph{#1}}}
	
%list style
\usepackage{enumitem} %for lists
\setlist[enumerate]{topsep=0.5ex,itemsep=-0.5ex,partopsep=1ex,font=\normalfont}%itemindent=1.5em



% theorem environments
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]   
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{construction}[theorem]{Construction}
\theoremstyle{remark}
%\newtheorem*{remark}{Remark}
\newtheorem{remarknumbered}[theorem]{Remark}
%\newtheorem*{speculation}{Speculation}
% remarks with different names
\makeatletter
\newtheoremstyle{remarknamedstyle}%
{\topsep}{\topsep}
{}{}
{\itshape}{.}
{0.5em}
{\thmname{\@ifempty{#3}{#1}\@ifnotempty{#3}{#3}}}
\makeatother
\theoremstyle{remarknamedstyle}
\newtheorem*{remark}{Remark}% here the second argument is the default name

% theorems with different names
\makeatletter
\newtheoremstyle{theoremnamedstyle}%
{\topsep}{\topsep}
{\itshape}{}
{\bfseries}{.}
{0.5em}
{\thmname{\@ifempty{#3}{#1}\@ifnotempty{#3}{#3}}}
\makeatother
\theoremstyle{theoremnamedstyle}
\newtheorem*{theoremnamed}{Theorem}% here the second argument is the default name
\crefname{theoremnamed}{Theorem}{Theorems}

% figures
\usepackage{wrapfig}
\usepackage{tikz,tikz-cd}
\usetikzlibrary{backgrounds}
\usetikzlibrary{arrows,arrows.meta}
\usetikzlibrary{shapes,shapes.geometric,shapes.misc}
\usetikzlibrary{intersections}
\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{background,edgelayer,nodelayer,main}
\tikzstyle{none}=[inner sep=0mm]
\tikzstyle{tikzfig}=[baseline=-0.25em,scale=0.5]
\tikzstyle{RRed_text}=[text={rgb,255: red,190; green,49; blue,26}]
\tikzstyle{dot_point}=[fill=black, draw=none, shape=circle, inner sep=1pt]
\tikzstyle{thick_dotted}=[-, dotted, thick]
\tikzstyle{thin_dotted}=[-, dotted]
\tikzstyle{green_open}=[-, fill={rgb,255: red,225; green,255; blue,235}, very thick]
\tikzstyle{green_cone}=[-, draw=none, fill={rgb,255: red,176; green,255; blue,176}, fill opacity=.5]
\tikzstyle{blue_cone}=[-, draw=none, fill={rgb,255: red,205; green,249; blue,255}, fill opacity=.34]
\tikzstyle{blue_open}=[-, fill={rgb,255: red,239; green,255; blue,255}, very thick]
\tikzstyle{yellow_opencone}=[fill={rgb,255: red,255; green,255; blue,220}, draw=none]
\tikzstyle{yellow_open}=[-, fill={rgb,255: red,255; green,255; blue,220}, fill opacity=1, very thick]
\tikzstyle{yellow_cone}=[-, draw=none, fill={rgb,255: red,255; green,244; blue,185}, fill opacity=.5]
\tikzstyle{yellow_cone_light}=[-, draw=none, fill={rgb,255: red,255; green,244; blue,185}, fill opacity=.2]
\tikzstyle{red_open}=[-, fill={rgb,255: red,255; green,228; blue,228}, very thick]
\tikzstyle{red_cone}=[-, fill={rgb,255: red,255; green,230; blue,230}, fill opacity=.5, draw=none]
\tikzstyle{red_dashed}=[-, fill={rgb,255: red,255; green,228; blue,228}, very thick, draw={rgb,255: red,71; green,26; blue,26}, dash pattern={{on 10pt off 2pt on 1pt off 2pt}}]
\tikzstyle{grey_open}=[-, fill={rgb,255: red,240; green,240; blue,240}, very thick]
\tikzstyle{grey_cone}=[-, draw=none, fill={rgb,255: red,218; green,218; blue,218}, fill opacity=.5]
\tikzstyle{real_line}=[-, ultra thick]
\tikzstyle{real_line_blue}=[ultra thick, draw={rgb,255: red,135; green,197; blue,255}, {|-|}]
\tikzstyle{real_line_red}=[ultra thick, draw={rgb,255: red,191; green,0; blue,3}, {|-|}]
\tikzstyle{real_line_yellow}=[ultra thick, draw={rgb,255: red,217; green,145; blue,0}, {|-|}]
\tikzstyle{real_line_grey}=[ultra thick, draw={rgb,255: red,171; green,171; blue,171}, {|-|}]
\tikzstyle{preimage_frames}=[->]
\newcommand{\tikzfig}[1]{{\tikzstyle{every picture}=[tikzfig]\input{#1.tikz}}}

